Improving Language Model Negotiation with Self-Play and In-Context Learning from AI Feedback

We study whether multiple large language models (LLMs) can autonomously improve each other in a negotiation game by playing, reflecting, and criticizing. We are interested in this question because if LLMs were able to improve each other, it would imply the possibility of creating strong AI agents with minimal human intervention. We ask two LLMs to negotiate with each other, playing the roles of a buyer and a seller, respectively. They aim to reach a deal with the buyer targeting a lower price and the seller a higher one. A third language model, playing the critic, provides feedback to a player to improve the player's negotiation strategies. We let the two agents play multiple rounds, using previous negotiation history and AI feedback as in-context demonstrations to improve the model's negotiation strategy iteratively. We use different LLMs (GPT and Claude) for different roles and use the deal price as the evaluation metric. Our experiments reveal multiple intriguing findings: (1) Only a subset of the language models we consider can self-play and improve the deal price from AI feedback, weaker models either do not understand the game's rules or cannot incorporate AI feedback for further improvement. (2) Models' abilities to learn from the feedback differ when playing different roles. For example, it is harder for Claude-instant to improve as the buyer than as the seller. (3) When unrolling the game to multiple rounds, stronger agents can consistently improve their performance by meaningfully using previous experiences and iterative AI feedback, yet have a higher risk of breaking the deal. We hope our work provides insightful initial explorations of having models autonomously improve each other with game playing and AI feedback.

==> GPTBargaining Arxiv/01_intro.tex <==
% \tushar{Some comments assuming this will be the main structure}

% P1.
% \hao{The success of AlphaGo Zero~\citep{silver2017mastering} demonstrates that modern AI systems can improve themselves with little human intervention, by continuously playing competition games with well-defined rules.
% This work studies its counterpart in natural language, and aims to investigate whether current large language models can successfully play a textual negotiation game and continuously improve their negotiation skills. reword ->
% }
% \yao{I feel like this reword is a bit of AlphaGo-centric which we may want to avoid (just like when we did complexity based prompting we wanted to minimize the influence of CoT even are a strongly inspired by them.)}
We study whether multiple Large Language Models (LLMs) can improve each other in a negotiation game with minimal human intervention, in the fashion of AlphaGo Zero~\citep{silver2017mastering}
where AI agents improve themselves 
% with little human knowledge 
by continuously playing competitive games under well-defined rules.
% \hao{
The answers to this research question have profound implications.
On the positive side, if the agents \emph{were} able to improve autonomously, strong agents might be created with  very few human annotations, which greatly saves the cost compared to today's data-hungry LLM training~\citep{chowdhery2022palm, hoffmann2022training}.
On the risky side, it also implies strong agents with limited human oversight~\citep{bowman2022measuring}. 
In this work, we ask two language models (a seller and a buyer) to bargain about a product. 
The seller is asked to sell the product at a higher price, while the buyer aims to purchase it at a lower price (Fig.~\ref{fig:method:method}A). 
After reaching a deal, 
% \hao{is this accurate? we never give feedback when they fail to reach a deal?}, 
% \yao{yes, future work}
we ask a third language model to play as the critic and give feedback to a player. 
Then we play the game again, asking the player to improve their strategy using AI feedback provided by the critic LLM. 

% \tushar{Might be worth highlighting that this is even less supervision than self-refine and other approaches, i.e., broader implications}
% \yao{Will do in the related work section}

\input{fig_02_method}

We choose the bargaining game because it
% simple \hao{i'd drop `simple,' since we immediately say it is not trivial in the next sentence}, 
comes with well-defined rules described in text, and a clear and measurable objective (a lower/ higher deal price) for strategic negotiation. 
% \hao{<- suggested rewording: ... because it comes with well-defined rules described in texts, and a clear and measurable objective (a lower or higher price that the product is sold at)}
Although the game seems easy at first glance, it requires non-trivial capabilities of the language models, as the model needs to: 
% \tushar{I have never seen periods after every number in a list when they are bracketed. Either choose brackets or periods.} \hao{+1}
(1) clearly understand and strictly follow the textual rules of the negotiation game 
% \hao{reworded};
(2) correspond to the textual feedback provided by the critic LM and improve based on it iteratively (see example feedback in Fig~\ref{fig:method:method}B);
(3) reflect upon the strategy and feedback over the long term and improve over multiple rounds. 
We will see that not all models we considered show all these abilities (Fig.~\ref{fig:method:method}C), and only
models that can (1) \textit{understand negotiation rules and strategies} (capable) and 
(2) \textit{respond to AI instructions} (well-aligned)
can continuously improve from AI feedback over multiple rounds (in our experiments, only \texttt{gpt-3.5-turbo}, \texttt{gpt-4}, and \texttt{claude-v1.3}) meet these requirements).
We have also tried more complicated textual games including board games and textual RPG games in the preliminary experiments, but they are more challenging for current agents to understand and follow the rules.

% \textit{strong} and \textit{well-aligned}\tushar{Best to drop these terms unless they can be defined based on some prior work. Instead just say "only a subset"} \hao{+ 1} models (in our experiments, \texttt{gpt-3.5-turbo}, \texttt{gpt-4}, and \texttt{claude-v1.3}) exhibit the ability of continuously improving from AI feedback over multiple rounds. 
% Generally, we observe that \textit{stronger} agents better \textit{understand negotiation rules and strategies}, and \textit{well-aligned} agents better \textit{respond to AI instructions}. 


% \hao{in addition to these points above, how about mentioning that in preliminary experiments we have tried asking them to play more complicated textual games including board games and textual RPG games, but they fail to understand and follow the rules. my reason for this is that our current framing can be pretty provocative and controversial to some readers; admitting the limitations of LLMs would clearly differentiate us from the "AGI spark" thing.}


% P2. Why we choose this game: because this is a minimum setting. More difficult cannot play game. Easier cannot draw meaningful conclusions.
% \tushar{This might be a hard claim and maybe doesn't have to be this strong. You could just say that we chose a game that is simple enough to evaluate an agent's ability to learn negotiation skills via self-play. Simpler or harder games could be used but we don't have to claim that its not possible or that they are less meaningful.} Though this is minimum, not all runs are successful, so still nontrivial.
% To perform this game, we require the model be able to: (1). role-playing dialog (2). reason about numbers (3). make decision on deal. \tushar{These are the abilities needed to play this game? Also could we connect this to the abilities being taught with AI feedback?}We will see that not all models exhibit these abilities. 

We call our approach \textit{In-Context Learning from AI Feedback} (ICL-AIF). 
% \hao{how about CLEAF? easier to pronounce}
% \yao{where does it come from ...}
Specifically, we use the feedback
% \hao{-> feedback?} 
from the AI critic as well as the previous rounds of dialog history as in-context demonstrations~\citep{brown2020language}.
By doing this, the critic's suggestions for improvements and the player's actual improvement in the previous rounds
% multiple rounds of the previous dialog
% \tushar{strategy is implicit. Might be better to use "dialog" or "negotiations" here.} \hao{+1} 
% and the suggestions for improvements 
effectively become the few-shot prompts for the next round of negotiation. 
We use in-context learning for two reasons:
% \hao{both of these two points below are basically saying we cannot afford fine-tuning and icl is the next best thing we can find. can we say something arguing that our setting is more realistic and better reflect real-world applications?}
% \yao{(1) says ICL is cheap and (2) says ICL has a theory}
(1) tuning large language models with reinforcement learning is prohibitively expensive~\citep{ouyang2022training, glaese2022improving} and the base model~\citep{OpenAI2023GPT4TR} may not be accessible to a wide range of the community; 
(2) in-context learning is recently shown to be closely related to gradient descent~\citep{dai2022can, akyurek2022learning, von2022transformers}, such that the conclusions we draw is fairly likely to generalize when one actually finetunes the model (if resources permit). 
One notable difference between our ICL-AIF and the mainstream Reinforcement Learning from Human Feedback (RLHF) is that in RL the reward is a \textit{scalar}~\citep{ouyang2022training, glaese2022improving} while in ICL the feedback is in \textit{natural language}. 
We study AI feedback (rather than rely on human intervention after each round) because it is more scalable and can allow models to self-improve automatically.

% We study AI feedback (instead of human feedback) because recent work shows that AI feedback can be comparable to human feedback~\citep{wu2021recursively, saunders2022self, bai2022constitutional} while being more scalable.\tushar{Hmm. this seems like you would rather use human feedback but ai feedback is more scalable. But you actually want the model to use AI feedback and not human feedback. So just a slight rephrasing: "We study AI feedback (rather than rely on human intervention after each round) since it is more scalable and can allow models to self-improve automatically.} \hao{+1. our whole point is AI agents improving themselves. }



% We discover multiple intriguing observations in our experiments: 
Our experiments lead to several intriguing findings:
(1) The requirements of our bargaining game effectively serve as a testbed for assessing the abilities of LLMs (Fig.~\ref{fig:method:method}C): although most models can do chitchat in a casual scenario, as of our experiment date (May 2023), \texttt{cohere-command}~\citep{cohere} model does not understand the rule of bargaining (Fig.~\ref{fig:exp:not_do_bargain}A), 
\texttt{ai21-jurassic}~\citep{jurassic} model does not respond to AI feedback (Fig.~\ref{fig:exp:not_do_bargain}B), \texttt{claude-instant-v1.0} can at most improve one round (Fig.~\ref{fig:method:multi_round}), and only \texttt{gpt-3.5-turbo}, \texttt{gpt-4}, and \texttt{claude-v1.3} can continuously improve over multiple rounds. 
(2) Models behave differently upon receiving feedback when playing different roles.
% vary in reaction\tushar{"reaction" doesn't really fit. "vary in their performance improvement"?} \hao{or, ``behave differently''}. 
Models playing the buyer role may be harder to improve than when in the seller role (Fig.~\ref{fig:exp:role_and_engine}). 
(3) It is indeed possible for strong agents like \texttt{gpt-4} to continuously improve meaningfully using previous experiences and online iterative AI feedback, yet the attempt to sell at a higher price (or buy at a lower price) comes with the risk of failing to reach a deal at all (Fig.~\ref{fig:method:multi_round_all_model}).
We further show evidence of the model being able to negotiation in a less
verbose but more strategic (thus more effective) way (Fig.~\ref{fig:exp:response_length}).
% suggesting future improvements about long-term planning and global optimization. \tushar{Why does planning help with preventing this specific negative outcome?} \hao{+1. besides, it seems we meant that LLMs need to be improved (on a vaguely-defined criteria), it might be misread and understood as our approach needs to be improved, which we should definitely avoid saying in the intro. i would just drop the "suggesting future ..." clause}
% Different models respond to feedback differently when playing different roles
Overall, we hope our work serves as a meaningful initiative for improving language models' negotiation in a game setting using AI feedback.  


==> GPTBargaining Arxiv/02_problem_statement.tex <==

\input{fig_02_do_bargain}
Our goal is to study whether LLMs can improve each other by playing a negotiation game and incorporating AI feedback, as shown in Fig.~\ref{fig:method:method}A.
We set the product being bargained as a balloon (and our results hold when changing the balloon to other items).
% \tushar{Just a curious thought: does the behavior change when you change the object? Most likely not, but it might be worth confirming that your findings are general.}. \hao{+ 1}
We use different combinations of backend LLM engines:
\texttt{cohere-command}~\citep{cohere}, AI21's \texttt{jurassic-2}~\citep{jurassic}, OpenAI's \texttt{gpt-3.5-turbo} and \texttt{gpt-4}~\citep{OpenAI2023GPT4TR}, Anthropic's \texttt{claude-instant-v1.0} (which supposedly matches \texttt{gpt-3.5-turbo}~\citep{chain-of-thought-hub}) and \texttt{claude-v1.3} (which is supposed to be slightly worse but close to \texttt{gpt-4}~\citep{chain-of-thought-hub}).
throughout our experiments, we \textit{provide feedback to improve only one} of the two players, while its rival receives no feedback, clears the negotiation history of previous rounds, and restarts. 
% In a multi-round game, we let the player that is being optimized to maintain the dialog history and AI feedback of all previous rounds, while always clearing its rival's dialog history (memory) in a new round. 
% This allows us to compare models with AI feedback over multiple rounds v.s. models with no feedback. 
% \hao{i can't parse this sentence: } 
We vary the engines for the model being improved while fixing its rival's engine to be \texttt{gpt-3.5-turbo}. 
Essentially, our game is \texttt{gpt-3.5-turbo} vs. all other engines.
We keep the LM engine behind the critic is always the same as the player it provides feedback to.
One example setting is a \texttt{gpt-4} seller playing against a \texttt{gpt-3.5-turbo} buyer, with a \texttt{gpt-4} critic.
After one round, the \texttt{gpt-4} critic provides feedback to the \texttt{gpt-4} seller such that the seller can improve in the next round while its rival \texttt{gpt-3.5-turbo} buyer clears its dialog history and restarts. 

\textbf{Process of the Game}\quad\quad 
% \hao{the paragraph title does not really match the content.} \hao{we should also emphasize that the seller should try to sell for a higher price by the rules. similar for the buyer's rule.}
% \hao{
Before the game begins, the rules of the negotiation game are explained to the models through textual instructions with the objective of selling/ buying at a higher/ lower price. 
We set the deal price to $[\$10, \$20]$ for easier evaluation, since other the deal price may vary in a wide range according to the observations from our preliminary experiments.
To achieve this, we hard code the seller to kick off the negotiation with ``This is a good balloon and its price is \$20.''
Similarly, the buyer always opens with ``Would you consider selling it for \$10?''
When both players strictly follow the game rules, the deal price would be between \$10 and \$20.
We let the models play multiple runs and measure the average deal price before and after AI feedback. 
During the game, the seller's output is used to prompt the buyer and vice versa, conditioning on the entire conversation history.
% rewording ->} 
% We explain the rule of bargaining to the seller and the buyer as the initial instructions of their prompt (which requires models' capability of understanding the rule). \hao{an example of the prompt explaining the rules would be helpful}
% Then we fix the seller's asking price to be \$20 by hard-coding the seller's opening as ``this is a good balloon and its price is \$20''.
% Similarly, we set the buyer's opening as 
% ``Would you consider selling it for \$10?''.
% This allows us to fix the price in [10, 20] for better evaluation (otherwise the deal price varies highly according to our preliminary experiments). 
% Then we prompt the seller model to generate an output text in response to the buyer. 
% The seller's response is fed as input to the buyer and its response is then fed back to the seller.
This process is repeated till a terminal state is reached.
Fig.~\ref{fig:method:do_bargain}A shows an example round.
% Also do all models have a chat mode?}. 
We define three game states:
(1) ON-GOING: the negotiation between the two players is still ongoing;
(2) DEAL: the negotiation has concluded and the two players have reached a deal; % reach a price they both agree on;
(3) NO DEAL: the players cannot agree on a price and have failed to reach a deal. 
To track the game states, we set an additional moderator 
% \hao{is this a fourth LM, or just the same one as the critic? we'd better clarify upfront if it is the former case.} 
(powered by a fourth LLM, in our case, \texttt{gpt-3.5-turbo}) to read the current dialog and classify the states (we will discuss more details about the moderator later). 
We measure the performance of the players based on the final deal price.
% \hao{add a sentence to clarify that for the seller, higher the better, and buyer lower the better?}


% \hao{we had some wording of ``self-reflecting'' in the abs/intro. does this mean we instruct the player ``What can you learn from the previous round to improve yourself?'' Would this be interesting to try?}
% \yao{We let the buyer to say ``I will improve over previous round''}
\textbf{Critic}\quad\quad 
% \hao{
A round is finished when the negotiation reaches a terminating state, either a DEAL or NO DEAL.
After each round, the critic LM is asked to provide constructive feedback to the player we aim to improve.
This player's dialog history from all past rounds and all feedback it has received are used to prompt the critic LM  (Fig.~\ref{fig:method:do_bargain}B).
The critic model is instructed to provide three suggestions to the player, in order to improve its negotiation strategies to achieve a more favorable price in the next game.
Before the next round, the player being improved receives the critic's feedback as a textual prompt, while its rival clears its negotiation history and restarts.
% rewording ->}
% After a game run
% \hao{"round" can be easily confused with a round of conversation.
% we should clarify that each game round is concluded after the negotiation has reached a terminating state},
% we use the player's, say the seller's, entire dialog history
% \hao{i would avoid the `memory' term. i'd be more concrete and say dialog/negotiation history} 
% (which includes the most recent round, and all previous rounds as well as their feedback) as the prompt for the critic (Fig.~\ref{fig:method:do_bargain}B).
% Then we instruct the critic to read the seller's memory and then provide three suggestions for the seller to sell the product at a higher price.
% This requires the seller's capability of improving from natural language feedback. 
% The same rule applies if the critic is helping the buyer, but recall that only one player is being improved while the other is fixed. 
% \hao{i can't follow why this sentence fits here, and can't parse the sentence in the brackets: } This allows us to measure the effectiveness using the final price (otherwise if two players are both optimized, their final price may stay the same). 





% \textbf{}. 

% Giving and receiving feedback is an emergent ability on models large and aligned well. -- 
% * Cite KYC paper saying models larger than 175B can be improve with language feedback 
% * In our early experiments we find GPT-3.5, GPT-4, Claude, and Bard-4.02 can use AI feedback, models weaker\tushar{By definition, models that can not do X ("use feedback" here) are weaker. So this seems like a trivial finding. Is there something more interesting that we can say other than "weaker"?} than them cannot
% * Being able to receive language feedback to improve themselves is a form of emergent ability, that emerges at (1). large enough model; (2). late alignment stage\tushar{new phrase. can you dumb it down?}. 
% [A figure showing LLM evolution stages, Bard-0315 is not well aligned but Bard-0402 is; GPT-3.5, GPT-4, Claude can do this. Other models cannot]

% \textbf{Why ICL-AIF}. 
% (1). in-context learning v.s. reinforcement learning;
% (2). AI feedback (when strong enough) similar to human feedback (but more scalable)
% (3). the ability of receiving AI feedback only exist when agents are aligned enough. 

% The Alignment Problem. [A figure show: human preference directly injecting to actor; injected to critic then actor; injected to meta-critic]

\textbf{The Moderator}\quad\quad 
The game state is classified by prompting a \texttt{gpt-3.5-turbo} moderator using few-shot demonstrations. 
The moderator reads the most recent four rounds (as well as in-context examples of different dialog states) and determines the state of the negotiation. 
Empirically, we found that four rounds of conversations are sufficient for the moderator to determine the negotiation state.
% -- confirmation of a final price and confirmation of a deal from both the players. 
One key challenge here is detecting no-deals as the model seems to be better at recognizing DEAL than NO DEAL.
% \hao{just say the DEAL label?}.
% The engineering challenge here is that there exist multiple false positives as the model is much better at recognizing deal than not deal (which is interesting yet unknown why). \tushar{A bit conversational. Change to "One key challenge here is detecting no-deals as the model seems to be biased towards predicting a deal".}
We mitigate this issue by playing multiple runs, inspect failure cases manually, and add them to the prompt with corrected labels. 
% incrementally adding false positive cases with corrected labels
% \tushar{as in you add actual false positives (negative examples with positive labels)? or add negative examples that are likely to be falsely labeled as positives?} 
% into the prompt as we play the game. \tushar{Why not add all of them in one go? Why incrementally?} \hao{+1. and how are these negative examples built?}
We find this method an effective side product recommend it as a technique for prompt optimization for generic classification tasks.
% \hao{i'd drop the second of of this sentence starting with "side product." it is hard for me to connect this to other general settings}

% \hao{is this paragraph below necessary? these relations are pretty obvious. it is unclear to me what else we are trying to say}\tushar{+1. Is it to contrast to related work?}
% \textbf{Relationship \hao{-> Relations} between Agents}\quad\quad
% The seller and the buyer compete with each other, 
% % We note that in our game setting, the relationship between the seller and the buyer is \textit{competitive}, 
% as one's gain means the other's loss. 
% Yet a player and its critic are \textit{cooperative}, as the critic is asked to provide better suggestions to improve the player, and the player should incorporate the critic's feedback. 
% We show examples of such cooperation in Fig.~\ref{fig:method:method}B, where the critic gives feedback like ``the power of silence'' and the buyer incorporates this strategy by playing ``\*pause\* ...'' in the next round. 

\textbf{Playing for Multiple Rounds}\quad\quad
Finally, we would like to explore whether the players can continuously improve from AI feedback in a game over multiple rounds.
Intuitively, the more rounds the players play, the more challenging to keep improving because the (already improved) price from the previous round becomes the baseline for the next round. 
In the experiments, we will show that only \texttt{gpt-4} can improve over 5 rounds while other models' improvements may saturate at about 3 rounds. 

% threshold.\tushar{a bit vague. "improvements generally saturate by XXth round"}  \hao{+ 1}
% \hao{should we mention somewhere that multiple games are played between each pair of rivals?}
% \yao{Done}


==> GPTBargaining Arxiv/03_related_work.tex <==
\textbf{Game Playing and AlphaGo Zero}\quad\quad
Our setting is strongly inspired by AlphaGo Zero~\citep{silver2017mastering} where two agents play the game of Go and improve each other with minimal human intervention.
Here we would like to explore its counterpart in natural language. 
Our work is similar to AlphaGo Zero in the sense that we also have AI agents (large language models) playing \textit{competitive} games (bargaining) and try to improve with little human supervision. 
Yet there is an important difference between our work and AlphaGo Zero: we have a third agent, \textit{the critic}, to give feedback helping its player to improve. This is a \textit{cooperative} relationship that does not exist in AlphaGo Zero.
On the NLP side, the closest related work is~\citet{lewis2017deal} where they have (small) RNN~\citep{chung2014empirical} language models to bargain, and our work can be viewed as a more developed version of them since we change the engine to be large language models.
In general, our work is broadly under the area of AI negotiation~\citep{chawla2021casino, chawla2021casino}, strategic reasoning~\citep{meta2022human}, and general game playing~\citep{silver2016mastering}. 

\textbf{Large Language Models as Generative Agents}\quad\quad
Large language models have demonstrated incredible multi-dimensional capabilities~\citep{wei2022emergent, OpenAI2023GPT4TR}, especially in complex reasoning~\citep{wei2022chain, qiao2022reasoning, fu2022complexity} and multi-round dialog~\citep{glaese2022improving, askell2021general, bai2022constitutional}, which serve as the foundation of this work. 
Our work is related to concurrent works like Generative Agents~\citep{park2023generative} and CAMEL~\citep{li2023camel} as they also study the behavior of LLMs in a multi-agent game setting. 
The core difference between our work and theirs is that we have a clear objective (the deal price) for the model to improve through competition and cooperation, while their work studies the generic social behavior of LLMs.


\textbf{Learning from AI Feedback}\quad\quad
Our method is also strongly inspired by constitutional AI~\citep{bai2022constitutional} as we both use AI feedback, while the difference is that our feedback is directly in natural language (not a scalar from a reward model). 
There are also related/ concurrent works demonstrating the effectiveness of natural language feedback~\citep{scheurer2022training, perez2022discovering, liu2023languages} and self-refinement~\citep{chen2023teaching, madaan2023self}. 
Our work further confirms the effectiveness of AI feedback in the strategic negotiation game setting.



% Large Language Models, Alignment, Emergent Abilities. Giving and receiving AI feedback is an emergent ability on when the model is large and mature enough

% AI feedback. Self-improvement. Why this is important 


% Language Games. Classic games, Stanford Generative Agents paper, Camel paper.

==> GPTBargaining Arxiv/04_experiments.tex <==

In our experiments, we consider three stages that gradually deepen our exploration of learning from AI feedback:
(1) We first set up the basics of the game (Sec.~\ref{ssec:basic_exps}), showing that only a few models can improve from AI critics, in which case AI feedback can be comparable (but more scalable) as human feedback.
Other models either do not understand/ follow the rule of bargaining, or cannot incorporate AI feedback for improvements. 
(2) Then we study the models’ behaviors when playing different roles (Sec.~\ref{ssec:llm_backend}).
We discover the intriguing result that buyers are in general harder to improve than sellers. 
(3) Finally, we study whether models can continuously improve over multiple rounds (Sec.~\ref{ssec:multiround_improvements}), and show a tradeoff of deal price versus success rate: although some models can continuously improve the deal price, it comes with a higher risk of breaking a deal. 
We further show evidence of negotiation in a more strategic way: both \texttt{gpt-4} and \texttt{claude-v1.3}'s responses become longer after multiple rounds of AI feedback (note that verbosity is a straightforward negotiation strategy), yet \texttt{gpt-4} is less verbose than \texttt{claude-v1.3} but achieves higher deal price and deal rate, meaning that its responses, although using fewer words, are more strategic and effective. 

% which indicates that future
% study may consider how to optimize the long-term return than the next-round deal price.

\subsection{Experiment Setup}
\label{ssec:exp_setup}
\input{fig_04_not_do_bargain}

\textbf{Model Engines}\quad\quad 
The minimum requirement for models to enter our game is that they should be a chatbot. 
All models we consider (\texttt{cohere-command}, AI21's \texttt{jurassic-2}, OpenAI's \texttt{gpt} and Anthropic's \texttt{claude}) can be accessed by API calls. 
Amoung them, \texttt{gpt-4} is the most expensive one and running 500 rounds of negotiation costs about \$120 and \texttt{gpt-3.5-turbo} costs about \$10. 
Other models are beta testing (as of May 2023) and do not charge money. 
For reference, the approximate rank of these models, from benchmarks like chain-of-thought hub~\citep{chain-of-thought-hub} and HeLM~\citep{liang2022holistic}, is that \texttt{gpt-4} and \texttt{claude-v1.3} are approximately similar, better than \texttt{gpt-3.5-turbo} and \texttt{claude-instant-v1.0}, and better than \texttt{cohere-command} and \texttt{j2-jumbo-instruct}. 
We will consider more models in the future, such as Google's PaLM-2~\citep{PaLM2}.

% API access. Prior rank. Price. Minimum requirement is models being a chatbot. More possible future

We let all models compete with \texttt{gpt-3.5-turbo}, effectively making it a baseline for all other models. 
We will show that, aligning with other concurrent model rankings~\citep{chain-of-thought-hub, liang2022holistic}, \texttt{gpt-3.5-turbo} is a middle-level powerful engine (worse than \texttt{gpt-4}, better than \texttt{claude-instant-v1.0}).
% \tushar{Do you mean that all other models are competing to better bargain with this base model? Basline would imply that you are going to compare the deal price of all models against gpt-3.5.}\tushar{Any way to justify this choice? Or indicate that the choice of the base model does not really matter?} 
For a given model engine (say \texttt{claude-v1.3}),
% we let it play the seller first (so \texttt{gpt-3.5-turbo} will be the buyer), then switch the role.\tushar{This seems like the order of running experiments which doesn't matter. Do you mean: "
we run it as the seller (with \texttt{gpt-3.5-turbo} as the buyer) and as a buyer (with \texttt{gpt-3.5-turbo} now as the seller)
% } 
We first let the models to play one round and manually inspect if they understand the rules of bargaining.
If they do,
% \tushar{how is this measured?}, 
we let them play two rounds to see if they could respond to AI feedback.
For the critic model, we set its engine the same as its player. 
We repeat the game 500 times to compute the average deal price before and after AI feedback. 
If they do improve one round, 
% \tushar{do ...?}, 
we let them play multiple rounds and see if they could continuously improve their strategy.
We repeat the game 200 times with 5 max rounds to compute the average deal price for each round.
% \tushar{how many max rounds?}. 
When decoding from the model engines, we use sampling with default temperature (1.0 for \texttt{gpt} and \texttt{claude}, 0.75 for \texttt{cohere} and 0.7 for \texttt{j2}).
% \tushar{Would that mean we may not be choosing the optimal, albeit greedy, generation for cohere and j2?}. 
% \yao{I believe temperature will not help}

% \textbf{Hyperparameters}\quad\quad 

\input{tab_04_human_baseline}

\textbf{Prompt Engineering}\quad\quad
% Most of this work's prompt engineering goes to the moderator \tushar{
In this work, we only had to manually optimize the prompts for the moderator  
% }
because the player may reach/ break a deal with very diverse expressions, and we would like to make sure the moderator correctly recognizes all of them.
As mentioned above, 
we identify the errors made by the moderator in identifying deals and keep adding them as in-context demonstrations until the model reaches a sufficiently high accuracy (about 90+ by manual inspection).
% we achieve this by progressively correcting and adding error cases as the in-context demonstrations, which we find very effective for prompt optimization.
% \tushar{Is this correct: 
% we identify the errors made by our prompt in identifying deals and keep adding them as in-context demonstration? Also when did you decide to stop?}
For the players and the critic, we do not do prompt engineering and keep the instructions the same for all engines (but the format may be different, e.g., \texttt{claude} requires two linebreaks before ``HUMAN:'' and \texttt{j2} requires two ``\#\#'' after each dialog round).
% \tushar{
Code and Prompts will be released publicly on publication. 
% ?} 


% \input{fig_04_baselines}



\subsection{Basic Experiments}
\label{ssec:basic_exps}

In this section, we first study the minimal requirements for models to participle in our game, namely (1) understanding the rule of bargaining and (2) responding to AI feedback. 
Then we consider basic comparison between AI and human feedback, showing that AI feedback can be comparable to human feedback, but more scalable. 


\input{fig_04_role_and_engine}

\textbf{Conversational ability does not guarantee ability to negotiate or learning from feedback}\quad\quad 
% \tushar{alternative title w/o these terms: Conversational ability does not guarantee ability to negotiate or learning from feedback.} 
% \yao{awesome!!}
We study whether conversational models can understand the rule of bargaining by manually checking  traces of the dialog, and found that \texttt{cohere-command} fails to understand the rules, as is shown in Fig~\ref{fig:exp:not_do_bargain}A. 
We observe that it does not realize what price is a better deal. 
For example, when playing seller, it rejects a proposal of \$10 but accepts \$8.
We also observe that AI21's \texttt{j2-jumbo-instruct} model, although understanding the rule of bargaining, cannot incorporate AI feedback, as is shown in Fig.~\ref{fig:exp:not_do_bargain}B.
Generally, when instructed with AI feedback, the model keeps the same strategy as before, without any improvements. 

After ruling out the \texttt{cohere-command} and \texttt{j2-jumbo-instruct} models, we consider 
% three stronger \tushar{
the three remaining
% } 
models: \texttt{gpt-3.5-turbo}, \texttt{claude-instant-v1.0} and \texttt{claude-v1.3}. 
For these three engines, we do not observe the problems in Fig.~\ref{fig:exp:not_do_bargain}.
% This means that these models are enough capable (such that they could understand the rule)\tushar{a bit tautological. Capable models are capable of negotiating.} and aligned (such that they could follow the AI feedback)\tushar{why is this the definition of aligned?}, ready to play our multi-round games. \tushar{
This means that these models can be used for our multi-round games.
% }

% \input{fig_04_example_techniques}
\textbf{AI Feedback can be comparable to human feedback}\quad\quad 
Now we consider some initial comparison between AI and human feedback. 
We emphasize that our goal is not to show which one is better -- a similar level of effectiveness would suffice our study (to see if LLMs can continuously improve through self-play and AI feedback). 
For the human feedback, we manually write done a pool of 10 suggestions.
Then we play 500 runs of the game, computing the deal price before and after feedback. 
After 500 runs, we compare the improvements after: 
(1) randomly sampling 3 suggestions from the predefined pool and 
(2) asking the AI critic to write down 3 suggestions. 
We note that this may underestimate the performance of human feedback, yet it would be unpractical to ask human to write done 3 suggestions for all 1500 runs (while AI feedback does not have this problem). 
The results are shown in Table~\ref{tab:exp:human_baseline} where we see that all three models (\texttt{gpt-3.5-turbo}, \texttt{claude-instant-v1.0} and \texttt{claude-v1.3}) exhibit comparable improvements over human and AI feedback. 


\input{fig_04_multiround}

\subsection{Behaviors of Different LLM Backend}
\label{ssec:llm_backend}
So far we have established that our game setting is valid for stronger LLM engines. 
Now we consider the detailed behavior comparisons using different engines for different roles. 
Specifically, we use \texttt{claude-instant-v1.0}, \texttt{claude-v1.3}, \texttt{gpt-3.5-turbo}, and \texttt{gpt-4} to play the seller/ buyer (against a \texttt{gpt-3.5-turbo} buyer/ seller respectively), then study the deal price distribution before/ after AI feedback (also recall that the AI critic is powered by the same engine as its player). 
The results are visualized in Fig.~\ref{fig:exp:role_and_engine}. When \texttt{claude-instant-v1.0} and \texttt{gpt-3.5-turbo} play the seller, they are able to improve their average deal price after AI feedback (Fig.~\ref{fig:exp:role_and_engine}A).
But when they play the buyer role, their average deal price does not improve, which indicates that buyers tend to be a harder role than sellers (Fig.~\ref{fig:exp:role_and_engine}B). 
Yet this observation does not hold for
% more powerful 
engines
% \tushar{more parameters? stronger performance on some tasks?} 
like \texttt{gpt-4} and \texttt{claude-v1.3}, as they can still improve from AI feedback even playing buyers. 
Overall, this set of experiments reveal the nuanced capability differences between the four engines we consider. 

% \subsection{Multiple Critics}

% \subsection{Multi-Agent Alignment}

\subsection{Towards Continuous Improvements from Iterative AI Feedback}
\label{ssec:multiround_improvements}

Now we unroll the game to multiple rounds and see if models can continuously improve from previous dialog history and iterative AI feedback. 
Specifically, we let \texttt{gpt-3.5-turbo}, \texttt{gpt-4}, \texttt{claude-instant-v1.0}, and \texttt{claude-v1.3} play as the seller/ buyer respectively against a rival powered by \texttt{gpt-3.5-turbo}. 
As mentioned before, the critic shares the same engine as the player it helps with. 
We play 200 runs of the game, and unroll each game to be 5 rounds. 
We compute the final deal price and the deal success rate and see if the price can be continuously improved. 


\input{fig_04_multi_round_all_models}

\input{fig_04_response_length}


Fig.~\ref{fig:method:multi_round} shows  \texttt{gpt-3.5-turbo} and \texttt{claude-instant-v1.0} playing different roles. 
For a given engine, improvements over one round may not necessarily extrapolate to multiple rounds, as we observe that \texttt{gpt-3.5-turbo} can improve over multiple rounds, but \texttt{claude-instant-v1.0} only improves at most one round. 

Now we consider the tradeoff between the tendency of achieving a higher deal price versus the rick of breaking a deal, as is shown in Fig~\ref{fig:method:multi_round_all_model}. 
We see that when playing sellers, all four model engines can improve over at least one round, but this comes at the cost of decreasing deal success ratio. 
When playing buyers, there are models that cannot improve (\texttt{claude-instant-v1.0}), or saturate over 3 rounds (\texttt{claude-v1.3}), while \texttt{gpt-4} and \texttt{gpt-3.5-turbo} can continuously improve, and \texttt{gpt-4} achieves better (lower) deal price and higher deal rate than \texttt{gpt-3.5-turbo}. 

Finally, we study how iterative AI feedback influences the language complexity used by the agents by plotting the average response length (measured in number of characters) after each round, as is shown in Fig.~\ref{fig:exp:response_length}. 
We see that both \texttt{claude-v1.3} and \texttt{gpt-4} become more verbose after iterative AI feedback with a continuously increasing response length. 
This is intuitive because being verbosity is a straightforward strategy in negotiation. 
Yet for \texttt{claude-v1.3}, the verbosity does not translate to better negotiation strategy, as its improvement saturates after three rounds (Fig.~\ref{fig:method:multi_round_all_model}B1). 
In comparison, \texttt{gpt-4}'s increase verbosity is more strategic, as it use less words than \texttt{claude-v1.3}, but achieves better deal price and deal success rate (Fig.~\ref{fig:method:multi_round_all_model}B). 
This observation serve as strong evidence that AI feedback improves players' response towards a word-tuned, strategic direction. 






==> GPTBargaining Arxiv/05_conclusions.tex <==
In this work, we study whether multiple large language models can autonomously improve each other in a negotiation game by role-playing and learning from AI feedback. 
Our experiments show that certain
models can indeed improve by
continuously playing competition games with iterative AI feedback, under well-defined rules in an AlphaGo Zero fashion. 
We also show the tradeoff between next-round price improvement and success rate, as a better deal price also comes with a higher risk of deal breaking. 
This suggests future research may consider global optimization for improving the overall gain over multiple rounds. 
We further show evidence of improved language from iterative AI feedback: in a multi-round game, one model may be less verbose than another, but be better word-tuned, thus more effective in getting a better deal.

We believe our results have profound implications for AI research:
on the positive side, it indicates the possibility of continuously improving language models with minimal human intervention.
% In particular, this approach does not require human data annotation. 
On the risky side, it might be more challenging to oversight the model behavior in our framework because models are acting autonomously, 
which calls for future alignment and safety research in the multi-agent game setting. 
Overall, we believe our work provides a meaningful initial exploration for large language models' learning from game-playing and iterative AI feedback.

==> GPTBargaining Arxiv/fig_02_do_bargain.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figures/do_bargain.pdf}
  \caption{ \label{fig:method:do_bargain}
  An example of playing the negotiation game and then improving from AI feedback. 
  \textbf{A}: \texttt{claude-instant-v1.0} plays the seller and \texttt{gpt-3.5-turbo} the buyer, bargaining about a balloon. 
  \textbf{B}: then we use a \texttt{claude-instant-v1.0} critic to provide feedback. 
  \textbf{C}: upon receiving the feedback, the seller improves its strategy based on the suggestions. Note that colored phrases like ``high quality latex and handcrafted by expert artisans'' correspond to previous AI feedback ``how rare and special it is''.
  We measure the final price as the proxy of the effectiveness of the strategy because the overall goal is to get a better price. 
  In this case, it improves from \$16 to \$17. 
  }
\end{figure*}


==> GPTBargaining Arxiv/fig_02_method.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figures/method_with_case.pdf}
  \caption{ \label{fig:method:method}
  Settings of our negotiation game.
  \textbf{A}. We ask two LLM agents to play a bargaining game as the seller and the buyer. Their goals are to sell/ buy the product at a higher/ lower price. 
  % \tushar{Minor: Add ellipses ... for round 1 and round 2 to indicate that the conversation does continue after the first two statements.} \hao{ + 1}
  After a round, we ask an AI critic, a third LLM,  to provide feedback to the player we want to improve. 
  Then we ask the player to improve their negotiation strategies based on the feedback.
  We repeat this process for multiple rounds and study if models can continuously improve. See Fig.~\ref{fig:method:do_bargain} for an example run.
  \textbf{B}. Bargaining techniques that we observed from the AI Critic and how the player incorporates these techniques into the negotiation strategy.
  \textbf{C}. Abilities that are required in our game (C2 - negotiation, C3 - AI feedback, and C4 - continuous improvements) classify models into different tiers. 
  We find out that only strong and well-aligned models (like \texttt{gpt-4} and \texttt{claude-v1.3}) can continuously improve from iterative AI feedback (see Fig.~\ref{fig:exp:not_do_bargain} for example models that do not exhibit these abilities).
  % \tushar{I love your mini-robot heads but might be worth dropping them here for readability.}]
  % \tushar{Also is this categorization empirical? E.g. If score(model1, task2) > threshold then model1 $\in$ B2? Might be worth mentioning this more clearly in the intro or figure.}\hao{+1. we need to be clear about the criteria. i remember even for gpt-4, it fails to follow rules sometimes?}
  }
\end{figure*}


==> GPTBargaining Arxiv/fig_04_baselines.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figures/baselines.pdf}
  \caption{ \label{fig:exp:baselines}
  Effectiveness of AI feedback compared to a constant baseline and a random human feedback baseline. After AI feedback the seller achieves better deal price. In addition, AI feedback exhibit the advantage of being more scalable. All agents use gpt-3.5-turbo backend. 
  ADD experiments on GPT-4 and Claude. 
  Change y-axis to be delta over initial price
  }
\end{figure*}


==> GPTBargaining Arxiv/fig_04_example_techniques.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figures/example_techniques.pdf}
  \caption{ \label{fig:exp:example_techniques}
  Bargaining techniques that we observed from the AI Critic and how the player incorporates these techniques into the negotiation strategy. \tushar{Very cool! Worth a intro figure. Which model(s) are these from?}
  }
\end{figure*}


==> GPTBargaining Arxiv/fig_04_multi_round_all_models.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figures/multi_round_all_model.pdf}
  \caption{ \label{fig:method:multi_round_all_model}
  Performance of GPT and Claude models in multi-round games and their success rate of getting a deal. 
  \textbf{A1} and \textbf{A2}: when playing the seller, most models can improve over multiple rounds. Yet higher prices also mean that it is more likely the seller may break the deal,
%   \hao{-> run away from a deal}, 
  as shown in the continuously decreasing curve of A2. 
  \textbf{B1} and \textbf{B2}: when playing buyer, \texttt{claude-instant-v1.0} cannot improve over multiple rounds while others can. 
  Again, a better buying price also comes with a higher chance of 
%   breaking the deal \hao{
  running away from a deal.
%   }. 
  We see that \texttt{GPT-4} achieves the best trade-off here: it gets the best price over multiple rounds with a higher success rate of reaching a deal. %maintaining a low deal break rate. 
%   \hao{i'd drop this. it doesn't look good to talk too much about future work in a submission}These results also indicate that future studies may consider how to optimize the long-term return than the next-round deal price. 
}
\end{figure*}


==> GPTBargaining Arxiv/fig_04_multiround.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figures/multi_round.pdf}
  \caption{ \label{fig:method:multi_round}
  In the multi-round setting, different engines have different behavior when playing seller/ buyer.
  Line plots are the average price over 200 runs and bar plots represent the price distribution.
  \textbf{A1} v.s. \textbf{B1}. When playing sellers, \texttt{gpt-3.5-turbo} can improve from AI feedback in multiple rounds, while \texttt{claude-instant-v1.0} only improves the first round.  
  \textbf{A2} v.s. \textbf{B2}. When playing buyers, \texttt{gpt-3.5-turbo} can improve in multiple rounds, whild \texttt{claude-instant-v1.0} cannot. 
}
\end{figure*}


==> GPTBargaining Arxiv/fig_04_not_do_bargain.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figures/not_do_bargain.pdf}
  \caption{ \label{fig:exp:not_do_bargain}
  Not all models can play bargaining. 
%   The capability of playing the negotiation game and improving from AI feedback only exists in models that are ``mature'' enough (strong and aligned). 
%   \hao{same concern as in the main text. i would just specify which models can improve and which cannot, instead of using terms such as machine, strong, or well-aligned}
  \textbf{A}. As of May 2023, the cohere model does not understand the rule of bargaining and agrees on irrational prices. 
  \textbf{B}. The AI21 Jurrasic-2 model, although understanding 
 the rule of bargaining, does not incorporate the feedback from the critic. 
 Since these models are consistently being updated, we include the timestamp and note future versions may have improved performance. 
 % \tushar{These examples are great. Can we empirically catch A without requiring manual analysis? I can imagine that we can catch B by seeing a negligible change in price after feedback.}
 % \yao{A bit hard ... }
}
\end{figure*}


==> GPTBargaining Arxiv/fig_04_response_length.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figures/response_length.pdf}
  \caption{ \label{fig:exp:response_length}
  The average response length increases as the model learns from multiple rounds. 
  Here we show examples of the seller's response when being asked the buyer's initial query ``Would you consider selling it for \$10?'' 
  After multiple rounds of negotiation, the seller's responses become more verbose and word-tuned. 
  Yet verbosity does not mean better strategy: \texttt{claude-v1.3} is more verbose (higher curve) than \texttt{gpt-4}, but it has a worse success rate and deal price (recall Fig.~\ref{fig:method:multi_round_all_model}).
  This indicates that \texttt{gpt-4}'s verbosity is more strategic. 
  }
\end{figure*}


==> GPTBargaining Arxiv/fig_04_role_and_engine.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=0.9\linewidth]{figures/role_and_engine.pdf}
  \caption{ \label{fig:exp:role_and_engine}
%   \hao{are the prices binned?}
  Binned deal price frequencies of 500 games,  before v.s. after feedback.
  % We simulate 500 runs \hao{runs -> games?} then draw the distribution of deal prices, before v.s. after feedback.
  Effective feedback should move the distribution towards a lower/ higher price range. 
  X-axis: intervals of deals from \$10 (buyers' initial price) to \$20 (sellers' asking price). Y-axis: the frequency of the price. \textbf{A} and \textbf{B}: for weaker agents like \texttt{claude-instant-v1.0} and \texttt{gpt-3.5-turbo}, improving from AI feedback as the seller is easier than as buyer. For sellers, AI feedback moves the deal distribution to a higher range (rightward), but does not move buyers' deal distribution much. Consequently, the change in average deal price when playing as buyers (-0.2 and -0.5) is clearly smaller than those as sellers (+1.0 and +1.7) 
  \textbf{C}. Stronger agents (\texttt{claude-v1.3}/ \texttt{gpt-4}), can still improve from AI feedback even as buyers, with larger changes in average deal price (-1.2 and -3.0). 
  % \tushar{Shift in distributions are not always easy to see. Would it be possible to add the average price within each image?} \hao{mean +- std }
  % \hao{also, can we change the y axis to percentage?}
  }
\end{figure*}


==> GPTBargaining Arxiv/tab_04_human_baseline.tex <==
\begin{table*}[t]
  \caption{
  \textbf{Seller performance} using AI feedback vs. randomly selected human feedback from a pre-defined pool. 
  % We use \texttt{gpt-3.5-turbo}/ \texttt{claude-instant-v1.0} as the seller.\tushar{you also have claude 1.3. Actually this sentence is unnecessary and could be dropped.} 
  Recall that the buyer is fixed to be \texttt{gpt-3.5-turbo} and has no access to previous rounds. 
  AI's feedback is comparable to human's, but is more scalable,
  % \tushar{pre-defined feedback is as scalable}), \yao{but you need to define it ..}
  as the two both induce similar price increases. 
  }
  \label{tab:exp:human_baseline}
  \centering
  \begin{tabular}{@{}l|ccc@{}}
      \toprule
       &  \bf GPT-3.5-Turbo &\bf  Claude-instant-v1.0 &\bf Claude-v1.3\\\midrule
      Before feedback  & 16.26  & 14.74  & 15.40 \\
      Random sampled human feedback & 16.83 (\blue{+0.57}) & 16.33 (\blue{+1.59}) & 16.89 (\blue{+1.49})\\ 
      AI feedback & 17.03 (\blue{+0.77}) & 15.98 (\blue{+1.24}) & 16.98 (\blue{+1.58})\\ 
      \bottomrule
  \end{tabular}
\end{table*}

==> fig_04_baselines.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figures/baselines.pdf}
  \caption{ \label{fig:exp:baselines}
  Effectiveness of AI feedback compared to a constant baseline and a random human feedback baseline. After AI feedback the seller achieves better deal price. In addition, AI feedback exhibit the advantage of being more scalable. All agents use gpt-3.5-turbo backend. 
  ADD experiments on GPT-4 and Claude. 
  Change y-axis to be delta over initial price
  }
\end{figure*}


==> fig_04_example_techniques.tex <==
\begin{figure*}[!t]
\small
  \centering
  \includegraphics[width=\linewidth]{figures/example_techniques.pdf}
  \caption{ \label{fig:exp:example_techniques}
  Bargaining techniques that we observed from the AI Critic and how the player incorporates these techniques into the negotiation strategy. \tushar{Very cool! Worth a intro figure. Which model(s) are these from?}
  }
\end{figure*}

